PureForest: A Large-Scale Aerial Lidar and Aerial Imagery Dataset for Tree Species Classification in Monospecific Forests

Knowledge of tree species distribution is fundamental to managing forests. New deep learning approaches promise significant accuracy gains for forest mapping, and are becoming a critical tool for mapping multiple tree species at scale. To advance the field, deep learning researchers need large benchmark datasets with high-quality annotations. To this end, we present the PureForest dataset: a large-scale, open, multimodal dataset designed for tree species classification from both Aerial Lidar Scanning (ALS) point clouds and Very High Resolution (VHR) aerial images. Most current public Lidar datasets for tree species classification have low diversity as they only span a small area of a few dozen annotated hectares at most. In contrast, PureForest has 18 tree species grouped into 13 semantic classes, and spans 339 km$^2$ across 449 distinct monospecific forests, and is to date the largest and most comprehensive Lidar dataset for the identification of tree species. By making PureForest publicly available, we hope to provide a challenging benchmark dataset to support the development of deep learning approaches for tree species identification from Lidar and/or aerial imagery. In this data paper, we describe the annotation workflow, the dataset, the recommended evaluation methodology, and establish a baseline performance from both 3D and 2D modalities.

==> classwise_perf_treesat.tex <==
\begin{figure}
\begin{tikzpicture}
\begin{axis}[
    width=1\linewidth,
    height=.3\textheight,
    ybar,
    bar width=.2cm,
    ylabel={Proportion (\%)}, %
    symbolic x coords={Deciduous oak,Evergreen oak,Beech,Chestnut,Black locust,Maritime pine,Scotch pine,Black pine,Aleppo pine,Fir,Spruce,Larch,Douglas},
    xtick=data,
    nodes near coords align={vertical},
    axis y line*=left, %
    xticklabel style={rotate=90,anchor=east},
    ymin=0,
    ymax=50,
    y label style={at={(axis description cs:+0.07,.5)},rotate=0,anchor=south},
    ]
\addplot [fill=lightgray] coordinates {(Deciduous oak,35.4) (Evergreen oak,16.5) (Beech,9.3) (Chestnut,2.7) (Black locust,1.7) (Maritime pine,5.6) (Scotch pine,13.5) (Black pine,5.3) (Aleppo pine,3.5) (Fir,0.6) (Spruce,3.0) (Larch,2.4) (Douglas,0.4)};
\legend{}; %
\end{axis}

\begin{axis}[
    width=1\linewidth,
    height=.3\textheight,
    axis y line*=right, %
    axis x line=none,
    ymin=0,
    ymax=100,
    nodes near coords,
    nodes near coords style={shift={(0ex,0.5ex)}},
    nodes near coords align={vertical},
    symbolic x coords={Deciduous oak,Evergreen oak,Beech,Chestnut,Black locust,Maritime pine,Scotch pine,Black pine,Aleppo pine,Fir,Spruce,Larch,Douglas},
    legend style={at={(0.5,-0.50)},
      anchor=north,legend columns=-1},
    ylabel={IoU (\%)}, %
    xticklabel style={rotate=90,anchor=east},
    ylabel near ticks, 
    yticklabel pos=right,
]
\addplot[mark=*,very thick, ForestGreen, text=black] coordinates {(Deciduous oak, 73.4) (Evergreen oak, 59.4) (Beech, 88.8) (Chestnut, 56.5) (Black locust, 58.1) (Maritime pine, 62.9) (Scotch pine, 58.6) (Black pine, 46.2) (Aleppo pine, 39.3) (Fir, 0) (Spruce, 85.8) (Larch, 50.6) (Douglas, 36.5)};
\end{axis}

\end{tikzpicture}
\caption{Class IoUs for the Lidar baseline model (green line), contrasted with class proportions in PureForest (grey bars).}
\label{fig:classwise_perfs}
\end{figure}

